Betty: An Automatic Differentiation Library for Multilevel Optimization

Gradient-based multilevel optimization (MLO) has gained attention as a framework for studying numerous problems, ranging from hyperparameter optimization and meta-learning to neural architecture search and reinforcement learning. However, gradients in MLO, which are obtained by composing best-response Jacobians via the chain rule, are notoriously difficult to implement and memory/compute intensive. We take an initial step towards closing this gap by introducing Betty, a software library for large-scale MLO. At its core, we devise a novel dataflow graph for MLO, which allows us to (1) develop efficient automatic differentiation for MLO that reduces the computational complexity from O(d^3) to O(d^2), (2) incorporate systems support such as mixed-precision and data-parallel training for scalability, and (3) facilitate implementation of MLO programs of arbitrary complexity while allowing a modular interface for diverse algorithmic and systems design choices. We empirically demonstrate that Betty can be used to implement an array of MLO programs, while also observing up to 11% increase in test accuracy, 14% decrease in GPU memory usage, and 20% decrease in training wall time over existing implementations on multiple benchmarks. We also showcase that Betty enables scaling MLO to models with hundreds of millions of parameters. We open-source the code at https://github.com/leopard-ai/betty.

==> design.tex <==
\section{Software Design}
\label{sec:software_design}

On top of the automatic differentiation technique developed in Section~\ref{sec:autodiff_mlo}, we take further steps to build an easy-to-use, modular, and maintainable programming interface for multilevel optimization within \textsc{Betty}.
Specifically, we break down MLO into two high-level concepts, namely 1) optimization problems and 2) the hierarchical dependencies among problems, and design abstract Python classes for each of them. From the dataflow graph perspective, each of these concepts respectively corresponds to nodes and edges. The architecture of \textsc{Betty} is shown in Figure~\ref{fig:diagram}.




\paragraph{Problem}
Each optimization problem $P_k$ in MLO is defined by the parameter (or module) $\theta_k$, the sets of the upper and lower constraining problems $\mathcal{U}_k$ \& $\mathcal{L}_k$, the dataset $\mathcal{D}_k$, the cost function $\mathcal{C}_k$, the optimizer, and other optimization configurations (\textit{e}.\textit{g} best-response Jacobian calculation algorithm, number of unrolling steps). The \texttt{Problem} class is an interface where users can provide each of the aforementioned components, except for the constraining problem sets, to define the optimization problem. We intentionally use a design where the constraining problem sets are provided, rather, by the \texttt{Engine} class. In doing so, users need to provide the hierarchical problem dependencies only once when they initialize \texttt{Engine}, and can avoid the potentially error-prone and cumbersome process of providing constraining problems manually every time they define new problems.
As for the remaining components, each one except for the cost function $\mathcal{C}_k$ can be provided through the class constructor, while the cost function can be defined through a \emph{``training\_step''} method. 
%\sang{Roughly speaking, \texttt{Problem} serves a similar purpose to PyTorch's \texttt{nn.Module}, but is used for representing an optimization problem instead of a neural network module.}

Once all the required components are provided, \texttt{Problem} implements a primitive for gradient-based optimization through a \emph{``step''} method. In detail, a \emph{``step''} method abstracts a one-step gradient descent update with four sub-steps: 1) data loading, 2) cost calculation, 3) gradient calculation, and 4) parameter update. \texttt{Problem} unrolls a predetermined number of gradient steps to approximate $\theta_k^*$ by running its \emph{``step''} method, and, when the optimization is done, calls the \emph{``step''} methods of upper level problems through lower-to-upper edges as discussed in Section~\ref{sec:data_flow}.

Furthermore, recall the differences between AID and ITD as reviewed in Section~\ref{sec:differentiaion_through_optimization}. ITD requires patching modules and optimizers to allow tracking of intermediate parameter states during optimization. To reflect such differences, we build two children classes, \texttt{ImplicitProblem} and \texttt{IterativeProblem}, by subclassing \texttt{Problem}.
The example usage of \texttt{Problem} is shown in Listing~\ref{lst:prob}.

\begin{lstlisting}[caption={\texttt{Problem} example},label={lst:prob}, language=Python]
class MyProblem(ImplicitProblem):
    def training_step(self, batch):
        # Users define the cost function here
        return cost_fn(batch, self.module, self.other_probs, ...)
        
config = Config(type="neumann", neumann_iterations=3, steps=5)
prob = MyProblem(name, config, module, optimizer, data_loader)
\end{lstlisting}
\vskip -7pt
Importantly, we provide a modular interface for users to choose different best-response Jacobian algorithms via a one-liner change in \texttt{Config}. This allows users without mathematical and programming expertise to easily and flexibly write a MLO code. All in all, our \texttt{Problem} and its \emph{``step''} method are similar in concept to PyTorch~\cite{paszke2019pytorch}'s \texttt{nn.Module} and its \emph{``forward''} method. Likewise, the parameter  in \texttt{Problem} before and after the \emph{``step''} method call corresponds to the input and the output of the neural network layer from the dataflow graph perspective.

\paragraph{Engine}
While \texttt{Problem} manages each optimization problem, \texttt{Engine} handles a dataflow graph based on the user-provided hierarchical problem dependencies. As discussed in Section~\ref{sec:data_flow}, a dataflow graph for MLO has upper-to-lower and lower-to-upper directed edges. We allow users to define two separate graphs, one for each type of edge, using a Python dictionary, in which keys/values respectively represent start/end nodes of the edge. When user-defined dependency graphs are provided, \texttt{Engine} compiles them and finds all paths required for automatic differentiation with a modified depth-first search algorithm. Moreover, \texttt{Engine} sets constraining problem sets for each problem based on the dependency graphs, as mentioned above. Once all initialization processes are done, users can run a whole MLO program by calling \texttt{Engine}'s run method, which repeatedly calls \emph{``step''} methods of lowermost problems. 
The example usage of \texttt{Engine} is provided in Listing~\ref{lst:engine}. 

\begin{lstlisting}[caption={\texttt{Engine} example},label={lst:engine}, language=Python]
prob1 = MyProblem1(...)
prob2 = MyProblem2(...)
depend = {"u2l": {prob1: [prob2]}, "l2u": {prob1: [prob2]}}
engine = Engine(problems=[prob1, prob2], dependencies=depend)
engine.run()

\end{lstlisting}
\vskip -7pt
To summarize, \textsc{Betty} provides a PyTorch-like simplified way of defining multiple optimization problems, which can scale up to large MLO programs with complex dependencies, as well as a modular interface for a variety of best-response Jacobian algorithms, without requiring mathematical and programming proficiency.
In its current version, most operations and low-level primitives of \textsc{Betty}, such as best-response Jacobian algorithms and module/optimizer patching for ITD, are implemented with PyTorch, which provides high efficiency with parallel GPU computing.
However, both \texttt{Problem} and \texttt{Engine} are largely abstract and implemented in a framework-agnostic way. Thus, we may consider supporting other frameworks including Tensorflow~\cite{abadi2016tensorflow} or JAX~\cite{frostig2018compiling} in the future.
%While both \texttt{Problem} and \texttt{Engine} are completely framework-agnostic, \textsc{Betty} only supports PyTorch in its current version, as most low-level primitives such as best-response Jacobian algorithms and module/optimizer patching for ITD are all implemented with PyTorch. In the future version, we may consider expanding the support for other frameworks including Tensorflow or JAX~\cite{jax2018github}.




==> design_full.tex <==
\section{Software Design}
\label{sec:software_design}

On top of the automatic differentiation technique developed in Section~\ref{sec:autodiff_mlo}, we take further steps to build an easy-to-use, modular, and maintainable programming interface for multilevel optimization within \textsc{Betty}.
Specifically, we break down MLO into two high-level concepts, namely 1) optimization problems and 2) the hierarchical dependencies among problems, and design abstract Python classes for each of them. From the dataflow graph perspective, each of these concepts respectively corresponds to nodes and edges. The architecture of \textsc{Betty} is shown in Figure~\ref{fig:diagram}.

\paragraph{Problem}
Each optimization problem $P_k$ in MLO is defined by the parameter (or module) $\theta_k$, the sets of the upper and lower constraining problems $\mathcal{U}_k$ \& $\mathcal{L}_k$, the dataset $\mathcal{D}_k$, the cost function $\mathcal{C}_k$, the optimizer, and other optimization configurations (\textit{e}.\textit{g} best-response Jacobian calculation algorithm, number of unrolling steps). The \texttt{Problem} class is an interface where users can provide each of the aforementioned components, except for the constraining problem sets, to define the optimization problem. We intentionally use a design where the constraining problem sets are provided, rather, by the \texttt{Engine} class. In doing so, users need to provide the hierarchical problem dependencies only once when they initialize \texttt{Engine}, and can avoid the potentially error-prone and cumbersome process of providing constraining problems manually every time they define new problems.
As for the remaining components, each one except for the cost function $\mathcal{C}_k$ can be provided through the class constructor, while the cost function can be defined through a \emph{``training\_step''} method. 
%\sang{Roughly speaking, \texttt{Problem} serves a similar purpose to PyTorch's \texttt{nn.Module}, but is used for representing an optimization problem instead of a neural network module.}

Once all the required components are provided, \texttt{Problem} implements a primitive for gradient-based optimization through a \emph{``step''} method. In detail, a \emph{``step''} method abstracts a one-step gradient descent update with four sub-steps: 1) data loading, 2) cost calculation, 3) gradient calculation, and 4) parameter update. \texttt{Problem} unrolls a predetermined number of gradient steps to approximate $\theta_k^*$ by running its \emph{``step''} method, and, when the optimization is done, calls the \emph{``step''} methods of upper level problems through lower-to-upper edges as discussed in Section~\ref{sec:data_flow}.

Furthermore, recall the differences between AID and ITD as reviewed in Section~\ref{sec:differentiaion_through_optimization}. ITD requires patching modules and optimizers to allow tracking of intermediate parameter states during optimization. To reflect such differences, we build two children classes, \texttt{ImplicitProblem} and \texttt{IterativeProblem}, by subclassing \texttt{Problem}.
The example usage of \texttt{Problem} is shown in Listing~\ref{lst:prob}.

\begin{lstlisting}[caption={\texttt{Problem} example},label={lst:prob}, language=Python]
class MyProblem(ImplicitProblem):
    def training_step(self, batch):
        # Users define the cost function here
        return cost_fn(batch, self.module, self.other_probs, ...)
        
config = Config(type="neumann", neumann_iterations=3, steps=5)
prob = MyProblem(name, config, module, optimizer, data_loader)
\end{lstlisting}
\vskip -7pt
Importantly, we provide a modular interface for users to choose different best-response Jacobian algorithms via a one-liner change in \texttt{Config}. This allows users without mathematical and programming expertise to easily and flexibly write a MLO code. All in all, our \texttt{Problem} and its \emph{``step''} method are similar in concept to PyTorch~\cite{paszke2019pytorch}'s \texttt{nn.Module} and its \emph{``forward''} method. Likewise, the parameter  in \texttt{Problem} before and after the \emph{``step''} method call corresponds to the input and the output of the neural network layer from the dataflow graph perspective.

\paragraph{Engine}
While \texttt{Problem} manages each optimization problem, \texttt{Engine} handles a dataflow graph based on the user-provided hierarchical problem dependencies. As discussed in Section~\ref{sec:data_flow}, a dataflow graph for MLO has upper-to-lower and lower-to-upper directed edges. We allow users to define two separate graphs, one for each type of edge, using a Python dictionary, in which keys/values respectively represent start/end nodes of the edge. When user-defined dependency graphs are provided, \texttt{Engine} compiles them and finds all paths required for automatic differentiation with a modified depth-first search algorithm. Moreover, \texttt{Engine} sets constraining problem sets for each problem based on the dependency graphs, as mentioned above. Once all initialization processes are done, users can run a whole MLO program by calling \texttt{Engine}'s run method, which repeatedly calls \emph{``step''} methods of lowermost problems. 
The example usage of \texttt{Engine} is provided in Listing~\ref{lst:engine}. 

\begin{lstlisting}[caption={\texttt{Engine} example},label={lst:engine}, language=Python]
prob1 = MyProblem1(...)
prob2 = MyProblem2(...)
depend = {"u2l": {prob1: [prob2]}, "l2u": {prob1: [prob2]}}
engine = Engine(problems=[prob1, prob2], dependencies=depend)
engine.run()

\end{lstlisting}
\vskip -7pt
To summarize, \textsc{Betty} provides a PyTorch-like simplified way of defining multiple optimization problems, which can scale up to large MLO programs with complex dependencies, as well as a modular interface for a variety of best-response Jacobian algorithms, without requiring mathematical and programming proficiency.
In its current version, most operations and low-level primitives of \textsc{Betty}, such as best-response Jacobian algorithms and module/optimizer patching for ITD, are implemented with PyTorch, which provides high efficiency with parallel GPU computing.
However, both \texttt{Problem} and \texttt{Engine} are largely abstract and implemented in a framework-agnostic way. Thus, we may consider supporting other frameworks including Tensorflow~\cite{abadi2016tensorflow} or JAX~\cite{frostig2018compiling} in the future.
%While both \texttt{Problem} and \texttt{Engine} are completely framework-agnostic, \textsc{Betty} only supports PyTorch in its current version, as most low-level primitives such as best-response Jacobian algorithms and module/optimizer patching for ITD are all implemented with PyTorch. In the future version, we may consider expanding the support for other frameworks including Tensorflow or JAX~\cite{jax2018github}.
